Comparative Analysis of Programming by Demonstration Methods: Kinesthetic Teaching vs Human Demonstration

Programming by demonstration (PbD) is a simple and efficient way to program robots without explicit robot programming. PbD enables unskilled operators to easily demonstrate and guide different robots to execute task. In this paper we present comparison of demonstration methods with comprehensive user study. Each participant had to demonstrate drawing simple pattern with human demonstration using virtual marker and kinesthetic teaching with robot manipulator. To evaluate differences between demonstration methods, we conducted user study with 24 participants which filled out NASA raw task load index (rTLX) and system usability scale (SUS). We also evaluated similarity of the executed trajectories to measure difference between demonstrated and ideal trajectory. We concluded study with finding that human demonstration using a virtual marker is on average 8 times faster, superior in terms of quality and imposes 2 times less overall workload than kinesthetic teaching.

==> content/03-kalipenSTARO.tex <==
\section{Kalipen - Active virtual marker}
\label{section:kalipen}

Building upon our previous work \cite{Maric_KDNO}, which presents a calibration method for a standard virtual marker, the primary objective of the Kalipen was to create a tool that facilitates efficient and easy robot programming. To achieve this objective, the tool was designed in a pen-like form, enabling intuitive and ergonomic handling. This streamlines the programing of tasks such as marking waypoints along the robot's path and identifying obstacles needed for collision-aware motion planning. Considering that robot paths often consist of multiple waypoints, the inclusion of a snapshot function was crucial, enabling the demonstrator to effortlessly store points of interest in a waypoints list with the press of a button. In addition, the shape of the Kalipen tip can be adjusted to suit different use cases and accommodate objects with varying shapes and forms that require measurement. Interested readers can refer to this in \cite{Maric_KDNO}. The tracking of the global position of the Kalipen relies on the \textit{Optitrack} motion capture system, which precisely tracks the reflective fiducials placed atop the Kalipen, providing a global pose with sub-millimeter accuracy. Special calibration procedures are implemented to ensure a proper understanding of the relationship between the tool tip (or tips) and the \textit{Optitrack} fiducials. 

\subsection{Hardware design}

The Kalipen is comprised of three main components: the modular tip, the body, and a set of passive IR reflective fiducials. In order to enable the trigger function for automatic storage of measured points, the pen's body was designed to include a button, feedback LEDs, battery and electronics with wireless communication functionality. The trigger button is placed on the bottom close to the tip, so the button can be triggered while holding the pen in the usual way. This makes it easy to precisely point and draw in 3D space.  

%\begin{figure}
%	\centering
%		\includegraphics[width=0.95\linewidth]{figures/marker.png}
%	\caption{Combining the functionalities of a wireless joystick and a virtual marker, we designed a prototype of an active virtual marker that can be used to program and deploy robotic systems.}
%	\label{fig:virtual_marker_device}
% \vspace{-0.5cm}
%\end{figure}

\begin{figure}
	\centering
		\includegraphics[width=0.95\linewidth]{figures/simple_pens.png}
	\caption{Simple pens with optitrack markers that were used for demonstrations. Left marker leaves trace. Right marker leaves no trace. }
	\label{fig:virtual_marker_device}
 \vspace{-0.5cm}
\end{figure}

Electronic components were put together using an \textit{Arduino}-based \textit{D1 Mini ESP32} micro-controller with \textit{Bluetooth} and \textit{Wi-Fi} functionalities. We opted for a Bluetooth connection to save energy.  The electronic device is equipped with a \textit{18650 Lithium-Ion} battery, along with a charging module. The device features an on/off switch and a single button used for the snapshot function. It is worth noting that more buttons can be easily added to the system.  Additionally, two LEDs are integrated to provide feedback to the user. The LEDs offer information such as the status of the Bluetooth connection, readiness of the device for measurement, button press acknowledgment, and charging status, among others. Communication is established using Bluetooth, which offers a 30 m range and efficient means of data transfer between the active pen and the computer. On the computer side, we use Bluetooth serial connection and a dedicated driver to enable interfacing with the ROS environment. 

% Technical parameters of the developed virtual marker are provided in Table \ref{table:device_performance}.

% \begin{table}[h!]
% \centering
%     \begin{tabular}{|c|c|} 
%          \hline
%          \textbf{Specification} & \textbf{Value}  \\ 
%          \hline\hline
%         Battery capacity: & $2.600 mAh$ \\ \hline
%         Weight: & 105 g (body of the marker) \\ \hline
%         Estimated battery time:  & aproxx. $20h$ \\ \hline
%         Wireless range: & up to $30 m$  \\
%          \hline
    
%     \end{tabular}
    
% \caption{virtual marker specification}
% \label{table:device_performance}
% % \vspace{-1.0cm}
% \end{table}

\subsection{Kalipen - Calibration}
\label{subsection:kalipen_calibration}

Given that the Optitrack motion capture system tracks the global pose $\mathbf{T}_W^I$ of the centroid of the fiducials placed on top of the Kalipen in world frame, precise calibration of the Kalipen tip becomes crucial. The calibration process involves deriving the relative transformation between the Kalipen tip and the Optitrack marker. Building upon our previous work, the calibration procedure varies depending on the specific type of tip being used. In this work, our primary focus is on a pointed tip type for the Kalipen, which serves various purposes including the measurement of global poses of points of interest and capturing the shape of objects. The pointed tip can be customized to have different levels of sharpness or roundness, allowing for precise point measurement or acquiring points by moving the tip across the surface of the object to be measured. While the specific tip shapes may vary, the underlying principles and steps of the calibration procedure remain the same. 

Taking into consideration the measurement of the pose of the fiducials centroid represented by $\mathbf{T}_W^I$, the calculation of the global pose of the Kalipen tip $\mathbf{T}_W^P$ is obtained using Eq. \ref{eq:tip_position}. The $\mathbf{T}_I^P$ represents the transformation between the fiducials centroid and the Kalipen tip.

\begin{equation}
    \mathbf{T}_W^P = \mathbf{T}_W^I \cdot \mathbf{T}_I^P .
    \label{eq:tip_position}
\end{equation}

The Kalipen calibration process consists of two steps. The first step involves calibration, establishing the spatial positioning of the Kalipen tip frame ($L_P$) with respect to the Optitrack marker frame ($L_I$). In the second step of the calibration process, the focus shifts to adjusting the orientation of the frame $L_P$. The goal is to align the $z_l$ axis of the Kalipen tip frame with the direction of the Kalipen tip itself, representing the approach vector. This alignment ensures that the orientation of the Kalipen tip is properly accounted for, allowing for accurate capturing of both the position and orientation of the robot waypoints and ensuring the proper functioning of the active pen system. 

% \begin{figure}%
% % \vspace{-0.5cm}
%     \centering
%     \subfloat[\centering Position calibration]{\includegraphics[width=.55\linewidth]{figures/denoted_point_calibration_setup.png} \label{fig:marker_calib_position} }%
%     \qquad
%     \subfloat[\centering Orientation calibration]{\includegraphics[width=.55\linewidth]{figures/denoted_orientation_calibration_setup.png} \label{fig:marker_calib_orientation}}%
%     \caption{The calibration process begins with dataset collection using specially developed tools. For the position calibration, the Kalipen tip is fixed at a specific location while the upper part moves and rotates. The global pose of the centroid of reflective fiducials, denoted as $\mathbf{T}_B^I$, is measured. The calibration then derives the transformation $\mathbf{T}_I^P$ to obtain the global pose of the Kalipen's tip, denoted as $\mathbf{T}_B^P$. Once the position calibration is completed, the next step is orientation calibration. In this step, the Kalipen is placed into a series of holes with known inclinations relative to the base link. The objective of the optimization process is to re-calibrate the pen transformation so that the measured vector $\mathbf{z}_p$ aligns with the reference vector $\mathbf{z}_{ref}$. This ensures accurate alignment of the marker's orientation.}%
%     \label{fig:marker_calibration}%
%     % \vspace{-0.5cm}
% \end{figure}

\begin{figure*}
	\centering
    \subfloat[\centering Position]{\includegraphics[width=.3\linewidth]{figures/denoted_point_calibration_setup.png} \label{fig:marker_calib_position} }%
    \qquad
    \subfloat[\centering Orientation]{\includegraphics[width=.3\linewidth]{figures/denoted_orientation_calibration_setup.png} \label{fig:marker_calib_orientation}}%
    \caption{The calibration process begins with dataset collection using specially developed tools. For the position calibration, the Kalipen tip is fixed at a specific location while the upper part moves and rotates. The global pose of the centroid of reflective fiducials, denoted as $\mathbf{T}_W^I$, is measured. The calibration then derives the transformation $\mathbf{T}_I^P$ to obtain the global pose of the Kalipen's tip, denoted as $\mathbf{T}_W^P$. Once the position calibration is completed, the next step is orientation calibration. In this step, the Kalipen is placed into a series of holes with known inclinations relative to the base link. The objective of the optimization process is to re-calibrate the pen transformation so that the measured vector $\mathbf{z}_p$ aligns with the reference vector $\mathbf{z}_{ref}$. This ensures accurate alignment of the marker's orientation.}
    \label{fig:marker_calibration}%
    \vspace{-0.4cm}
\end{figure*}

\subsubsection{Position calibration} process begins with dataset recording, where the Kalipen tip $\mathbf{T}_\mathrm{W}^{\mathrm{P}}$ is fixed at a specific point in the world reference frame $\mathbf{L}_W$, while the reflective fiducial part is moved and rotated throughout the space. The motion capture system tracks the pose of the fiducials centroid $\mathbf{T}_\mathrm{W}^{\mathrm{I}}$ and generates a calibration dataset of $N$ points. The optimization problem is formulated in Eq. \ref{eq:marker_opti_pos}, aiming to find the optimal translation $\mathbf{P}^\ast \in \mathbb{R}^{3 \times 1}$ as the translation component of the transformation matrix $\mathbf{T}_\mathrm{I}^{\mathrm{P}}$. The objective is to minimize the global distance discrepancies between the transformed points obtained using Eq. \ref{eq:tip_position}  across the entire calibration dataset. Fig. \ref{fig:marker_calib_position} provides a graphical illustration of the dataset generation. During the dataset recording, occlusion of fiducials can occur, particularly during fast movements, resulting in potential outliers within the dataset. To address this issue, a special clustering process was employed to eliminate outliers. Further details about the dataset filtering and optimization procedure can be found in our previous work \cite{Maric_KDNO}.

\begin{equation}
  \mathbf{P}^\ast = \argmin\limits_{\mathbf{P}} \sum_{\mathit{i}=1}^{\mathrm{N}} \sum_{\mathit{j}=1}^{\mathrm{N}} ||{\mathbf{T}_{\mathrm{O}, \mathit{i}}^\mathrm{I} \cdot \mathbf{T}_\mathrm{I}^{\mathrm{P}} - T_{\mathrm{O}, \mathit{j}}^\mathrm{I} \cdot \mathbf{T}_\mathrm{I}^{\mathrm{P}}}|| .
  \label{eq:marker_opti_pos}
\end{equation}

\subsubsection{Orientation calibration} step is an additional procedure that complements the position calibration and enables the full utilization of the Kalipen, particularly in scenarios where both the position and orientation are important. An example of such a scenario is Programming by Demonstration, where the robot needs to be shown not only where to pick up an object but also how to orient its grip. For the orientation calibration, a specially designed tool is used, as depicted in Fig. \ref{fig:marker_calib_orientation}. The tool comprises a series of $r$ holes, each having a predetermined orientation with respect to the reference frame of the motion capture system. The dataset collection process involves positioning the Kalipen tip in each hole of the tool in a defined order. Once the Kalipen is placed in a hole, it is rotated around the axis of the hole to capture a series of $N$ different poses of $\mathbf{T}_\mathrm{W}^{\mathrm{I}}$. 

The orientation calibration is formulated as an optimization problem, as defined in Eq. \ref{eq:line_opti_angle}.
\begin{equation}
     [\Psi^\ast, \Theta^\ast, \Phi^\ast]  = \argmin\limits_{P^\ast}\sum_{i=1}^{r} \sum_{j=1}^{N} \left \Vert \frac{\mathbf{z}_{ref, i} \cdot \mathbf{z}^{[\Psi^\ast, \Theta^\ast, \Phi^\ast]}_{i, j}}{||\mathbf{z}_{ref, i}|| \cdot ||\mathbf{z}^{[\Psi^\ast, \Theta^\ast, \Phi^\ast]}_{i, j}||} \right \Vert .
    \label{eq:line_opti_angle}
\end{equation}
The objective is to modify the rotational part of the transformation matrix $\mathbf{T}_\mathrm{I}^{\mathrm{P}}$ in order to align the measured vector $z_p$ with the reference vector $z_{\mathrm{ref}}$. The other vectors, $x_p$ and $y_p$, are not considered due to the axial-symmetric design of the pointed tip. Due to the nature of rigid body rotation being a part of the SO(3) group, it can be uniquely defined using minimal three parameters. Therefore, we have chosen to utilize the yaw-pitch-roll Euler notation to determine the optimal rotation $[\Psi^\ast, \Theta^\ast, \Phi^\ast]$. Similar to the position calibration, outlier filtering based on clustering is performed. Further details regarding the dataset filtering and the optimization procedure can be found in our previous work \cite{Maric_KDNO}. Finally, the Kalipen coordinate system is aligned in a way that the button aligns with the $y_p$ axis of the pen. This is important to make the user aware of the actual pose of the pen. 

As a result of the presented calibration procedures, the Kalipen is capable of measuring and marking points in the global reference frame with submillimeter accuracy and orientation precision of up to 1 degree in approach axis. This level of precision enables the Kalipen to effectively support various applications, such as Programing by Demonstration or object measurement, where precise positioning and orientation are crucial. 

% \subsection{Kalipen - Deployment}

% Deploying robots in any setting requires one to create a robotic task, denoted as ${\mathscr T}_r$. The robotic task ${\mathscr T}_r$ compromises a set of trajectories ${\mathscr T}_{i=1\dots N} \in {\mathscr T}_r$, where each trajectory is a series of time-dependent waypoints, represented by $w_p(t)$ ${\mathscr T}_{i} = \{ w_{p}(t):   t \in [0, T_i]\}$. To ensure collision-free motion, it is essential to create a virtual representation of the robot's workspace ${\mathscr W}_r$. This representation outlines the workspace boundaries and identifies various obstacles. 

% Here we will describe several procedures one can follow to sketch the robot's task and workspace utilizing the Kalipen device, eliminating the need to tediously measure and model their surroundings.  A schematic view of the capturing process is depicted in Fig. \ref{fig:box_capturing}. These uses highlight the versatility and practicality of the virtual marker in achieving accurate calibration and enhancing safety in robot operations. 

% \begin{figure}
% 	\centering
% 		\includegraphics[width=0.9\linewidth]{figures/bounding_box_new.png}
% 	\caption{The figure illustrates two possible applications of the virtual marker. The first is the calibration of the robot's base-link to the motion capture system, achieved through the known 3D model of the robot base and pointcloud obtained by drawing along its surface with the pen. The second application involves defining the collision objects in motion planning scene. The pen is used to measure four points for defining the box in the robot's planning scene. }
% 	\label{fig:box_capturing}
% \end{figure}

% \subsubsection{Point measurement}
% Optitrack continuously tracks the Kalipen's position in 3D space. This, coupled with the calibration $\mathbf{T}_I^P$, enables precise capture of points in Cartesian 3D space, defined by the following equation:

% \begin{equation}
%      \mathbf{p} =  \left[x \quad y \quad z \quad q_x \quad q_y \quad q_z \quad q_w \right] \in \mathbb{R}^{1 \times 7},  
%      \label{eq:point_P}
% \end{equation}
% \noident where the Kalipen tip position is denoted as $\mathbf{p}_p =  \left[x \quad y \quad z \right] \in \mathbb{R}^{1 \times 3}$, while the orientation of the Kalipen tip is expressed in quaternion form as $\mathbf{p}_q = \left[q_x \quad q_y \quad q_z \quad q_w \right] \in \mathbb{R}^{1 \times 4}$. This enables the user to show the waypoints or define obstacles by drawing freely whilst simultaneously collecting points. 


% \subsubsection{Add box procedure}

% To virtualize a priori unknown obstacles, or to define the boundaries of the robot's workspace we propose drawing on obstacles surrounding the robot, representing them as boxes. Establishing obstacle boundaries involves selecting points in a counter-clockwise direction around one side of the box. If capturing the fourth point isn't possible, users can manually specify the desired height $h$ perpendicular to the captured points' plane.



% \subsubsection{Add mesh procedure}
% Additionally, we introduce a user-friendly method for localizing known objects by drawing its shape with a Kalipen. This approach is well-suited for pinpointing specific objects within the robot workspace, especially those accurately modeled or robot parts (e.g., a known 3D model of the robot base or links). Initially, we convert a CAD model of the object into a point cloud. Subsequently, this model is matched to a scan of the actual object, obtained as a point cloud using the tracked Kalipen

% Preprocessing involves voxelizing both the object model and scan at similar resolutions and computing Fast Point Feature Histograms (FPFH) for correspondence \cite{rusu2009fast}. To find the initial transformation between the two clouds, the Sample Consensus Prerejective method is applied iteratively until a predefined fit threshold is achieved \cite{buch2013pose}. The transformation is further refined using the Iterative Closest Point (ICP) algorithm \cite{arun1987least}.

% The end result of the matching process is the pose of the 3D mesh, localized in the Optitrack coordinate frame. The mesh is then loaded in the MoveIt planning scene using \textit{addMesh()} function and providing it with the pose of the mesh.

\subsection{Kalipen - Deployment} % short version

Deploying robots in any setting requires one to create a robotic task, denoted as ${\mathscr T}_r$. The robotic task ${\mathscr T}_r$ compromises a set of trajectories ${\mathscr T}_{i=1\dots N} \in {\mathscr T}_r$, where each trajectory is a series of time-dependent waypoints, represented by $w_p(t)$ ${\mathscr T}_{i} = \{ w_{p}(t),   t \in [0, T_i]\}$. To ensure collision-free motion, it is essential to create a virtual representation of the robot's workspace ${\mathscr W}_r$. This representation outlines the workspace boundaries and identifies various obstacles. 

The Kalipen device serves various purposes, streamlining the process of mapping robot tasks and surroundings without the need for extensive measurements or modeling. Shown in Fig. \ref{fig:box_capturing}, its applications range from marking obstacles by pinpointing key geometric points for bounding boxes to user-friendly localization of known 3D objects by tracing their shapes. Despite its versatile uses, our primary focus in this work revolves around its key application: a human-friendly Human-Robot Interface (HRI) for capturing robotic task waypoints.

\begin{figure}
	\centering
		\includegraphics[width=0.9\linewidth]{figures/bounding_box_new.png}
	\caption{The figure illustrates two possible applications of the virtual marker. The first is the calibration of the robot's base-link to the motion capture system, achieved through the known 3D model of the robot base and pointcloud obtained by drawing along its surface with the pen. The second application involves defining the collision objects in motion planning scene. The pen is used to measure four points for defining the box in the robot's planning scene. }
	\label{fig:box_capturing}
\end{figure}

The point measurement process relies on Optitrack continuously tracking the Kalipen's pose in 3D space. This, in conjunction with the calibration matrix $\mathbf{T}_I^P$, ensures accurate capture of points in Cartesian 3D space, as defined by the following equation:

\begin{equation}
     \mathbf{p} =  \left[x \quad y \quad z \quad q_x \quad q_y \quad q_z \quad q_w \right] \in \mathbb{R}^{1 \times 7},  
     \label{eq:point_P}
\end{equation}

\noident where the Kalipen tip position is denoted as $\mathbf{p}_p = \left[ x \quad y \quad z \right] \in \mathbb{R}^{1 \times 3} $, while the orientation of the Kalipen tip is expressed in quaternion form as $\mathbf{p}_q = \left[q_x \quad q_y \quad q_z \quad q_w \right] \in \mathbb{R}^{1 \times 4}$. This enables the user to show the waypoints or define obstacles by drawing freely whilst simultaneously collecting points. 

% \subsubsection{Bounding boxes}

% \subsubsection{Localization using the Kalipen}


==> content/depr_01-introduction.tex <==
\section{Introduction}

Since introduction of robots, number of the ones installed in factory settings increases steadily. One of the most common and most used robots now days, in academia and industry, are robot manipulators. Robot manipulators can execute wide variety of different tasks, and they have been major factor in accelerating industrial automation. Despite their widespread use, standard robot manipulators present various challenges, ranging from the complexity to program up to almost complete lack of human-robot interaction (HRI) possibility. They are typically programmed using pre-programming methods for a specific task, undertaken by trained robotic engineers. However, this approach poses challenges, as these engineers may lack a comprehensive understanding of the specific tasks the robot needs to perform. 

In response to these challenges, there has been a shift in industrial demand towards collaborative robot manipulators \cite{grau2020_robots_in_industry}. Their collaborative capabilities, facilitating close human-robot interaction, can be used in various ways. Not only do they allow the operator and robot to share a workspace safely, but they also enable the operator to easily program the robot. Since the introduction of cobots, substantial efforts have been made in the Programming by Demonstration use case, wherein the operator kinesthetically guides the cobot's body directly to demonstrate how to perform specific tasks. This approach has generated considerable excitement \cite{Omkar2023_hype_cobots}, fostering expectations that cobots can be easily adopted in almost any situation. Yet, even with all the technologies that make it easy and safe to control the cobot, it can make the person feel a bit uneasy. This discomfort might lead the person to show the robot how to do things in a way that might not be the best. It's important to recognize situations where this method doesn't work well, especially for delicate tasks like delicate sanding, micro-drilling, putty plastering and similar activities.

In this paper, we will present Programming by Demonstration (PbD) when using specially developed virtual marker, and collaborative robot manipulator Franka Emika Panda. We believe that employing newer and simpler interfaces for demonstration can make it easier for people to start using robot manipulators. This applies to both collaborative and standard industrial manipulators, which are capable of performing various tasks when programmed properly. To support our claim, we conducted a user-experience survey where individuals were asked to demonstrate a simple drawing task with both a robot and a virtual marker. Main contributions of this paper are two fold. \textit{First contribution is introduction of the virtual marker, smart-pen paired with motion capture system  for task demonstration. Second contribution are results of the conducted user study which support our initial claims that new interfaces for HRI have potential to further adoption of the robot manipulators even with unskilled labor-force.}





% Since introduction of robots, number of the ones installed in factory settings increases steadily. One of the most common and most used robots now days, in academia and industry, are robot manipulators. Robot manipulators can execute wide variety of different tasks, and they have been major factor in accelerating industrial automation. One of the main challenges when using robot manipulators, presents itself in difficulty of human robot interaction (HRI). Most of the interaction is done through conventional programming which requires certain amount of expertise and knowledge. 

% Besides programming, newer robotic arms offer specialized interfaces in form of the rugged touchscreens where users can program certain trajectories or pick-and-place operations. More often than not, incorporating robot manipulator in factory settings, requires careful planning, financial and operational-wise. Besides planning, it requires collaboration between multiple people, ones who will implement it, and ones who will use it. In order to facilitate wider and easier adoption of the robot manipulators in factories, there exists need to create new ways to interact and program with robot manipulators. 

% In this paper, we will present Programming by Demonstration (PbD) when using special smart pen called Kalipen, and force interaction with Franka Emika robot manipulator. We argue that using newer and simpler interfaces for demonstration can facilitate easier adoption of the robot manipulators, especially collaborative ones, who are technically able to execute wide variety of tasks with proper demonstration. Main contributions of this paper are two fold. \textit{First contribution is introduction of the Kalipen, smart-pen paired with motion capture system  for task demonstration. Second contribution are results of the conducted user study which support our initial claims that new interfaces for HRI have potential to further adoption of the robot manipulators even with unskilled labor-force.}

\begin{figure}
	\centering
		\includegraphics[width=0.99\linewidth]{figures/exp_sketch.png}
	\caption{The experimental setup for the user-experience study comprised a motion capture system, specially developed virtual markers, and the collaborative robot \textit{Franka Emika Panda}. Participants were tasked with drawing simple images using both the virtual marker and the robot. Subsequently, user-experience, task load, and task evaluation were assessed through a questionnaire and task analysis.}
	\label{fig:exp_sketch}
 \vspace{-0.5cm}
\end{figure}

%TODO: Add VR/AR argument

Paper is divided in seven Sections. Section \ref{section:related_work} presents related work and how our work differentiates from existing PbD techniques. In section \ref{section:virtual_pen} we present virtual marker, with it's hardware design, and calibration methods. Section \ref{section:methodology} derives methodology used to enable smart functionality and what requirements we satisfied in order to conduct non-biased user study. In section \ref{section:experiments} we present results of our experiments. In \ref{section:conclusion} we conclude paper with most important findings and planned future work. 
%TODO: 
% - Add sources that support claims 
% - find resources to support claims of different programming interfaces


%In the learning phase, demonstrations are collected and segmented into action representations. Different methods, such as kinesthetic teaching \cite{Tykal2016_Kinesthetic} or tele-operation \cite{Zhang2018_VR}, can be used. In our prior work \cite{Maric_ENDORSE}, we explored kinesthetic teaching, guiding the robot's flange for a task involving delicate grinding of complex-shaped composite materials in aircraft manufacturing. It's worth noting that operator-guided robot demonstrations, while capturing complex motions, may be biased due to operator discomfort. Following the learning phase, the representation phase involves robot movement mapping and execution. Various approaches include probabilistic models \cite{Calinon2009}, data-driven AI models \cite{Scherzinger2019Contact}, and the increasingly popular Dynamic Movement Primitives (DMP) \cite{pastor2011_ICRA_DMP} in recent years.

% In the learning phase, demonstrations are gathered and segmented into action representations, forming an assembly tree that outlines the sequence of actions. Different methods, such as kinesthetic teaching \cite{Tykal2016_Kinesthetic} or tele-operation \cite{Zhang2018_VR}, can be employed for this stage. We previously explored the kinesthetic teaching approach in our work \cite{Maric_ENDORSE}, where the operator guided the robot's flange to demonstrate a specific task involving delicate grinding of complex-shaped composite materials used in aircraft manufacturing. It is noteworthy that while operator-guided robot demonstrations allow for the capture of complex motions for a specific task, the operator's performance may be biased due to discomfort in such an environment. Following the learning phase, the representation phase encompasses robot movement mapping and robot execution. Various representation approaches are available, including probabilistic models \cite{Calinon2009}, data-driven AI-based models \cite{Scherzinger2019Contact}, and the increasingly popular Dynamic Movement Primitives (DMP) \cite{pastor2011_ICRA_DMP} in recent years.



%In a notable Programming by Demonstration (PbD) application, Wang et al. \cite{Wang2023} introduced a robotic insertion task approach using visual servoing. Robot is able to recreate highly precise insertion task just by observing human doing it once. In our prior work \cite{maric_case_drilling}, we applied a similar method for deep micro-hole drilling, using a motion capture system instead of visual servoing. Following to that in \cite{maric2024_dmp} we extended our previous work by superimposing our methods with carefully designed and executed user study. Ajaykumar et al. \cite{ajaykumar2023} proposed a PbD system incorporating kinesthetic teaching and different modalities, like gaze and speech. Using multimodal PbD can lead to overtrust and automation bias in the long term, which is why it makes sense to explore HRI through PbD with different modalities of kinesthetic teaching and virtual marker demonstration. Steinmetz et al. \cite{steinmetz2019} suggested task-level PbD, useful for introducing collaborative robots in small and medium-sized enterprises. Main difference compared to ours approach is that they use kinesthetic teaching coupled with on-line semantic skill recognition algorithm which enables untrained operators to demonstrate certain task.

% Main contributions of this paper are two fold. 
%\textit{First contribution is the introduction of the virtual marker, smart-pen paired with motion capture system for the easy and intuitive, passive, task demonstration. Second 


%We have chosen simple drawing task for demonstration purposes because there is requirement to follow certain path whilst applying pressure on the surface.  Such patterns are also widely used in real world for tasks like painting, welding etc. The chosen drawing task diverges from specific and delicate industrial skills, ensuring that a broad range of participants possesses sufficient knowledge to perform it.

\vspace{-0.1 cm}
